SGD Finds then Tunes Features in Two-Layer Neural Networks with near-Optimal Sample Complexity: A Case Study in the XOR problem

In this work, we consider the optimization process of minibatch stochastic gradient descent (SGD) on a 2-layer neural network with data separated by a quadratic ground truth function. We prove that with data drawn from the $d$-dimensional Boolean hypercube labeled by the quadratic ``XOR'' function $y = -x_ix_j$, it is possible to train to a population error $o(1)$ with $d \:\text{polylog}(d)$ samples. Our result considers simultaneously training both layers of the two-layer-neural network with ReLU activations via standard minibatch SGD on the logistic loss. To our knowledge, this work is the first to give a sample complexity of $\tilde{O}(d)$ for efficiently learning the XOR function on isotropic data on a standard neural network with standard training. Our main technique is showing that the network evolves in two phases: a $\textit{signal-finding}$ phase where the network is small and many of the neurons evolve independently to find features, and a $\textit{signal-heavy}$ phase, where SGD maintains and balances the features. We leverage the simultaneous training of the layers to show that it is sufficient for only a small fraction of the neurons to learn features, since those neurons will be amplified by the simultaneous growth of their second layer weights.

==> sections/old.tex <==
\section{Phase 2 Old}
At the beginning of Phase 2, we divide the neurons into ``good'' neurons and ``bad neurons". On the good neurons, we will have fine grained control over their evolution throughout this phase. On the ``bad neurons'', we will use the fact that they can't grow more an exponential rate.

\begin{definition}[Good Neurons for Phase 2]
Let $\mathcal{G}$ be the set of neurons at such that:
\begin{enumerate}
    \item $\wsig^{(t + T_1)} = \zeta_1 d^{-1}\exp((1 + o(1))/\sqrt{2\pi}t - \alpha t)\on{sign}(\wsig^{(T_1)})$.
    \item $|\wopp^{(t + T_1)}| \leq \zeta_1 d^{-1}\exp((1 + o(1))/\sqrt{2\pi}t - 2\alpha t)$.
    \item $\|\wpe^{(t + T_1)}\| = \zeta_2\exp(-(\alpha \pm o(1)) t)$.
    % \item $ |\wsig^{(t + T_1)}| \geq |\wopp^{(t + T_1)}|\exp((1/\sqrt{2\pi} + o(1))t)$.
\end{enumerate}
for some $\zeta_1 \in \exp(\pm\Theta(\log\log\log(d)))$ and $\zeta_2 = \Omega(1/log(d)), o(1)$.
\end{definition}
\begin{definition}[Mediocre Neurons for Phase 2]
Let $\cM$ be the set of neurons at such that:
\begin{enumerate}
    \item $|\wsig^{(t + T_1)}| \leq \zeta_1 d^{-1}\exp((1 + o(1))/\sqrt{2\pi}t - \alpha t)$.
    \item $|\wopp^{(t + T_1)}| \leq \zeta_1 d^{-1}\exp((1 + o(1)/\sqrt{2\pi}t - 2\alpha t)$.
    \item $\|\wpe^{(t + T_1)}\| = \zeta_2\exp(-(\alpha \pm o(1)) t)$.
    % \item $ |\wopp^{(t + T_1)}| \leq \zeta_1 d^{-1}\exp((1 + o(1))/\sqrt{2\pi}t - \alpha t)\on{sign}(\wsig^{(T_1)})$.
\end{enumerate}
for some $\zeta_1 \in \exp(\pm\Theta(\log\log\log(d)))$ and $\zeta_2 = \Omega(1/log(d)), o(1)$.
\end{definition}
Note that $\cM$ is a super-set of $\cG$. In $\cM$, it is possible that $|\wopp| > |\wsig|$ (in fact $|\wsig|$ can be arbitrarily small), but $|\wopp|$ still cannot be too large - it grows at a most at an exponential rate $\alpha$ smaller than that of $\wsig$ in $\cG$.

We defined $\mathcal{B}$ to be the remaining set of neurons. 

Let $M$ be some large constant. Phase 1 guarantees that $\mathbb{P}_{\hrho_{T_1}}[\hw \in \cG] \geq 1 - \frac{1}{M}$ and $\mathbb{P}_{\hrho_{T_1}}[\hw \in \mathcal{B}] \leq d^{-M}$ for some sufficiently large $M$, and that $\mathbb{E}_{\hrho_{T_1}}[\|\hw\|^2\mathbf{1}(\hw \in \mathcal{B})] \leq d^{-M}$.


The core of this proof the following inductive lemma. We define the following inductive hypothesis.
\begin{definition}[Phase 2 Hypothesis]\label{def:hyp2}
    $\mathbb{P}_{\hrho_{t + T_1}}[\hw \in \mathcal{B}] \leq d^{-M}$ and $\mathbb{E}_{\hrho_{t + T_1}}[\|\hw\|^2\mathbf{1}(\hw \in \mathcal{B})] \leq d^{-M}\exp(4t)$. Suppose also that $\mathbb{P}_{\hrho_{t + T_1}}[\hw \in \cG] \geq 1 - \frac{1}{M}$.
\end{definition}

Let $\eps = \alpha/1000$, and let $T_2 = \sqrt{2\pi}(1 - \eps)\log(d)$.
\begin{lemma}[Phase 2 Inductive Step]\label{lemma:inductive}
Suppose for some $t \leq T_2$, the hypothesis in Defn~\ref{def:hyp2} holds.

Then $\eta \leq 0.1$, and $n \geq d(\log\log(d))^2\log(d)$, with probability at least $1 - d^{-M}$, we have the following:
 \begin{enumerate}
     \item For all $\hw^{(t + T_1)} \in \mathcal{G}$, $\hw^{(t + \eta + T_1)} \in \mathcal{G}.$
     \item For all $\hw^{(t + T_1)} \in \mathcal{M}$, $\hw^{(t + \eta + T_1)} \in \cM.$
     \item $\mathbb{E}_{\hrho_{t + \eta + T_1}}[\|\hw\|^2\mathbf{1}(\hw \in \mathcal{B})] \leq d^{-M}\exp(4(t + \eta)).$
 \end{enumerate}
\end{lemma}

Before proving Lemma~\ref{lemma:inductive}, we make the following observations about implications of the inductive hypothesis. For $z \in \{\pm e_1, \pm e_2\}$, let
\begin{align}
    A_{z} := \mathbb{E}_{\hrho}[\sigma(y(z)a(w)w^Tz)].
\end{align}
We abuse notation and for $v = cz$, for a constant $c$, we define $A_{v} = A_z$.
\begin{claim}\label{claim:inductive}
If Defn~\ref{def:hyp2} holds at some time $t$, we have
    \begin{enumerate}
        \item $B_t := \mathbb{E}_{\hrho_t}[|a(w)|\|w\|)] = o(1)$. 
        \item $\mathbb{E}_{\hrho_t}[\|w_{1:2}\|^2] = o(1)\mathbb{E}_{\hrho_t}[\|\hwpe\|^2]$.
        \item $\mathbb{E}_{\hrho_t}[\|w_{1:2}\|^2] = \frac{\zeta}{d}\exp((1 + o(1))/\sqrt{2\pi}t - 2\alpha t)$.
        \item $\mathbb{E}_{\hrho_t}[\|\hwpe\|^2] = \exp(-2\alpha(1 + o(1))t)$.
        \item $A_z \leq \frac{\zeta_1}{\sqrt{d}}\exp((1 + o(1))/\sqrt{8\pi}t - 2\alpha t)$ for all $z \in \{\pm e_1, \pm e_2\}$
    \end{enumerate}
\end{claim}
\begin{proof}
Simple computation.
\end{proof}

Our main tool in proving Lemma~\ref{lemma:inductive} are the next  two lemmas, concerning the growth of the signal and orthogonal components respectively. Finally, we have a lemma showing that with high probability, the error due to a SGD step with $n = d\log(d)(\log\log(d))^2$ data points is small enough to ignore. Together, these lemmas suffice to show Lemma~\ref{lemma:inductive}.

\begin{lemma}[Phase 2 Signal]\label{lemma:phase2signal}
For any $w$, we have
\begin{align}
    \mathbb{E}_{P}\left[\frac{d}{dt}\wsig^2\right] \in \frac{1}{\sqrt{2\pi}}\left(1 \pm \epsilon_2\right)\wsig^2 \pm |a(w)\wsig|\Theta\left(A_{\wsig}\right).,
\end{align}
    where 
\begin{align}
    \epsilon_2 = \Theta\left(B_t^2 +  \frac{|\wsig| + |\wopp|}{|\wpe| + |\wsig|}\right),
\end{align}

Further, we have 
\begin{align}
    \mathbb{E}_{P}\left[\frac{d}{dt}\wopp^2\right] \in \frac{1}{\sqrt{2\pi}}\left(-1 \pm \epsilon_2\right)\wopp^2 \pm |a(w)\wopp|\Theta\left(A_{\wsig}\right).
\end{align}
Thus assuming the inductive hypothesis, if $w \in \cG$ we have 
\begin{align}
    \mathbb{E}_{P}\left[\frac{d}{dt}\wsig^2\right] = \frac{1}{\sqrt{2\pi}}\left(1 \pm o(1)\right)\wsig^2.
\end{align}
Further, for all $w \in \cM$, we have
\begin{align}
    \mathbb{E}_{P}\left[\frac{d}{dt}\wopp^2\right] \leq \frac{\zeta_1}{d}\exp\left(\left(\frac{1}{\sqrt{2\pi}} + o(1)\right)t -2\alpha t\right)\exp(-2\alpha t),
\end{align}
and 
\begin{align}
    \mathbb{E}_{P}\left[\frac{d}{dt}\wsig^2\right] \leq \frac{1}{\sqrt{2\pi}}\left(1 \pm o(1)\right)\wsig^2.
\end{align}

% $\mathbb{E}_{P}\left[\frac{d}{dt}\hw_2^2\right] \leq \frac{1}{2}\mathbb{E}_{P}\left[\frac{d}{dt}\hw_1^2\right]$.

\end{lemma}

\begin{lemma}[Phase 2 Orthogonal]\label{lemma:phase2orth}
Without regularization, if $\|\hrho\|^2 \leq B_t \leq 0.2$, we have for an individual neuron:
\begin{align}
    \mathbb{E}_{P}\left[\frac{d}{dt}\|\hwpe\|^2\right] \in \pm \Theta(1)a(\hw)\|\hwpe\|\left(\frac{\|w_{1:2}\|}{\|w_{1:2}\| + \|\hwpe\|} + \mathbb{E}_{\hrho}[|a(w)|\sigma(\|w_{1:2}\|)]\right).
\end{align}

Thus assuming the inductive hypothesis of Phase 2 and that $\|\hw_{1:2}\| = o(1)\|\hwpe\|$ (which in particular holds for any $\hw \in \cM$), we have
\begin{align}\label{eq:perp}
\frac{d}{dt}\mathbb{E}[\|\hwpe\|^2] = o(1)\mathbb{E}[\|\hwpe\|^2].
\end{align}
\end{lemma}

\section{Phase 3 Old}

Phase 3 is similar to Phase 2, but because we run it for less time, we can me more course in our estimates of the evolution of $w_{1:2}$ and $\wpe$ in this phase. Thus we define $\mathcal{G}$ and $\cM$ in a slightly different way, to allow more deviation in the growth of the neurons. 

There are two main differences in the analysis in Phase 3:
\begin{enumerate}
    \item Since $|\wsig| > |\wpe|$ sometimes, we can only bound the exponential growth rate of $\wsig$ up to constant factors, as opposed to to the exact correct constant, as in Phase 2.
    \item Our analysis of $\|\wpe\|$ needs to use a different proof approach when $|\wsig| > |\wpe|$. Further, we can never show that $\|\wpe\|$ gets smaller that $\|\wopp\|$.
\end{enumerate}
The analysis of $\wopp$ is the same as in Phase 2.
\begin{definition}[Good Neurons for Phase 3]
Let $\mathcal{G}$ be the set of neurons at such that:
\begin{enumerate}
    \item $|\wsig^{(t + T_1 + T_2)}| = d^{-1}\exp((1 + o(1))/\sqrt{2\pi}T_2 - \alpha (T_2 + t) + c t)\on{sign}(w_{sig}^{(T_2)})$, where $c \in [1/20, 20]$.
    \item $|\wopp^{(t + T_1 + T_2)}| \leq d^{-1}\exp((1 + o(1))/\sqrt{2\pi}t - 1.5\alpha t)$
    \item $\|\wpe^{(t + T_1 + T_2)}\| = \max\left(d^{o(1)}\exp(-\alpha (t + T_2)), d^{\Theta(\eps)}\sup_{s \leq t}w_{opp}^{(T_1 + T_2 + s)}\right)$.
\end{enumerate}
\end{definition}
\begin{definition}[Mediocre Neurons for Phase 3]
Let $\cM$ be the set of neurons at such that:
\begin{enumerate}
    \item $|\wsig^{(t + T_1 + T_2)}| \leq d^{-1}\exp((1 + o(1))/\sqrt{2\pi}T_2 - \alpha (T_2 + t) + c t)\on{sign}(w_{sig}^{(T_2)})$, where $c \in [1/20, 20]$.
    \item $|\wopp^{(t + T_1 + T_2)}| \leq d^{-1}\exp((1 + o(1))/\sqrt{2\pi}t - 1.5\alpha t)$
    \item $\|\wpe^{(t + T_1 + T_2)}\| = \max\left(d^{o(1)}\exp(-\alpha (t + T_2)), d^{\Theta(\eps)}\sup_{s \leq t}w_{opp}^{(T_1 + T_2 + s)}\right)$.
\end{enumerate}
for some $\zeta_1 \in \exp(\pm\Theta(\log\log\log(d)))$ and $\zeta_2 = \Omega(1/log(d)), o(1)$.
\end{definition}

Let $M$ be some large constant. Phase 1 guarantees that $\mathbb{P}_{\hrho_{T_1}}[\hw \in \cG] \geq 1 - \frac{1}{M}$ and $\mathbb{P}_{\hrho_{T_1}}[\hw \in \mathcal{B}] \leq d^{-M}$ for some sufficiently large $M$, and that $\mathbb{E}_{\hrho_{T_1}}[\|\hw\|^2\mathbf{1}(\hw \in \mathcal{B})] \leq d^{-M}$.


The core of this proof the following inductive lemma. We define the following inductive hypothesis.
\begin{definition}[Phase 3 Hypothesis]\label{def:hyp3}
    $\mathbb{P}_{\hrho_{t + T_1}}[\hw \in \mathcal{B}] \leq d^{-M}$ and $\mathbb{E}_{\hrho_{t + T_1}}[\|\hw\|^2\mathbf{1}(\hw \in \mathcal{B})] \leq d^{-M}\exp(4t)$. Suppose also that $\mathbb{P}_{\hrho_{t + T_1}}[\hw \in \cG] \geq 1 - \frac{1}{M}$.
\end{definition}

Recall that $\eps = \alpha/1000$, $T_2 = \sqrt{2\pi}(1 - \eps)\log(d)$, and let $T_3 := 20\eps \log(d)$.

\begin{lemma}[Phase 3 Inductive Step]\label{lemma:inductive_3}
Suppose for some $t \leq T_2$, the hypothesis in Defn~\ref{def:hyp3} holds.

Then $\eta \leq 0.1$, and $n \geq d(\log\log(d))^2\log(d)$, with probability at least $1 - d^{-M}$, we have the following:
 \begin{enumerate}
     \item For all $\hw^{(t + T_1)} \in \mathcal{G}$, $\hw^{(t + \eta + T_1)} \in \mathcal{G}.$
     \item For all $\hw^{(t + T_1)} \in \mathcal{M}$, $\hw^{(t + \eta + T_1)} \in \cM.$
     \item $\mathbb{E}_{\hrho_{t + \eta + T_1}}[\|\hw\|^2\mathbf{1}(\hw \in \mathcal{B})] \leq d^{-M}\exp(4(t + \eta)).$
 \end{enumerate}
\end{lemma}

Our main tool in proving Lemma~\ref{lemma:inductive} are the next  two lemmas, concerning the growth of the signal and orthogonal components respectively. Finally, we have a lemma showing that with high probability, the error due to a SGD step with $n = d\log(d)(\log\log(d))^2$ data points is small enough to ignore. Together, these lemmas suffice to show Lemma~\ref{lemma:inductive}.

\begin{lemma}[Signal Phase 3]
For any $w \in \cG$,
    \begin{align}
    \mathbb{E}_{P}\frac{d}{dt}\mathbb{E}_{\hrho}[\sigma'(a(\hw))\hw_1\sigma(\hw_1)] \geq \frac{1}{20}\mathbb{E}_{\hrho}[\sigma'(a(\hw))\hw_1\sigma(\hw_1)].
 \end{align}
 \mg{Todo: add upper bound too, and perhaps phrase more generally}
\end{lemma}

\mg{To control $\wopp$, we will use the lemma from Phase 2, since nothing should change)}
\begin{lemma}[Phase 3 Orthogonal]\label{lemma:phase3orthogonal}
For any $M \geq 1$, we have
\begin{align}
    \mathbb{E}_P\left[\frac{d}{dt}\|\hwpe\|^2\right] \leq \begin{cases}
        M\|\hwpe\|^2\Theta\left(P_t + \mathbb{E}_{\hrho}[|a(w)|\sigma(\|w_{1:2}\|)]\right) & \|\hwpe\| \geq \frac{1}{M}|\hw_1|\\
        0 & |\hw_2| \leq \|\hwpe\| \leq \frac{1}{M}|\hw_1|\\
        a(\hw)\|\hwpe\|\exp(B_t^2)\left(\mathbb{E}_{\hrho}[|a(w)w^T\xi|] + \exp(-M^2)\right) & \|\hwpe\| \leq |\hw_2|.
    \end{cases}
\end{align}

\mg{Need to make an equivalent of this lemma for neurons in $\cM$, which might be a bit tricky for the second bullet, since now we can have $\wopp > \wsig$, so $\wpe$ can be growing, but hopefully not too fast. }
\end{lemma}



\section{Phases Revised}

% \subsection{Phase 4}

% \begin{definition}[Phase 4 Inductive Hypothesis]
% For a tolerance parameter $\zeta$, suppose the following holds:
% \begin{enumerate}
%     \item All but a $\zeta$ fraction of the network is supported on neurons that are $\zeta$-close to $\pm e_1$ or $\pm e_2$, in the proper signal direction.
%     \item The network is $2\zeta$-balanced, ie $$    \sup_{z_1, z_2 \in \{\pm e_1, \pm e_2\}} \frac{|A_{z_1}^{(t)} - A_{z_2}^{(t)}|}{\min(A_{z_i}) + 1} \leq 2\zeta$$
% \end{enumerate}
    
% \end{definition}

% \begin{lemma}
% Suppose the phase 4 inductive hypothesis holds at time $t$. Then after one step, the inductive hypothesis still holds, and we have

% $B \geq (1 + 0.01\eta\exp(-B))B$, where $B = \min(A_{z_i})$.
% \end{lemma}
% \begin{proof}
% Consider any data-point $x = z + \xi$, and wlog assume $|z_1| > |z_2|$ so that $y(z) = 1$.


% Then \mg{in expectation over $\xi$...would have to do this more formally}
% \begin{align}
%     f(x) \in |z_1|A_{z_1} - |z_2|A_{z_2} \pm 2\zeta(B + 1),
% \end{align}
% and so 
% \begin{align}
%     \ell'_{\rho}(x) &= \exp(-(|z_1|A_{z_1} - |z_2|A_{z_2} \pm 2\zeta(B  + 1)))\\
%     &= \exp(-B(|z_1| - |z_2|) \pm 2(B + 1)\zeta(1 + \|z\|))\\
%     &\in \exp(-B(|z_1| - |z_2|)(1 \pm 2(B + 1)\zeta(1 + \|z\|))
% \end{align}

% Thus for any any neuron $w$ with $|w^Te_1| \geq (1 - \zeta)\|w\|$, we have 
% \begin{align}
%     \mathbb{E}_x[\ell_{\rho}'(x)\sigma'(x^Tw)x_{1:2}] &= \mathbb{E}_{\xi}\mathbb{E}_z[\ell_{\rho}'(\xi + z)\sigma'(\xi^Tw + z^Tw)z]\\
%     &\in \mathbb{E}_z[\ell_{\rho}'(z)\sigma'(z^Tw)z] + \Delta_1\\
%     &\in  \mathbb{E}_z[\exp(-y(z)(A_{z_1}|z_1| + A_{z_2}|z_2|)))\sigma'(z^Tw)z] + \Delta_1 + \Delta_2
% \end{align}
% where
% \begin{align}
%     \Delta_1 &= \mathbb{E}_{\xi}\mathbb{E}_z[\left(\ell_{\rho}'(\xi + z)\sigma'(\xi^Tw + z^Tw) - \ell_{\rho}'(z)\sigma'(z^Tw)\right)z]\\
%     &= \mathbb{E}_{\xi}\mathbb{E}_z[\ell_{\rho}'(\xi + z) - \ell_{\rho}'(z))\sigma'(\xi^Tw + z^Tw)z] + \mathbb{E}_{\xi}\mathbb{E}_z[\ell_{\rho}'(z)(\sigma'(z^Tw) - \sigma'(\xi^Tw - z^Tw))z]\\
%     &\leq \Theta\left(\zeta (B + 1) \mathbb{E}_z\exp(-y(z)f_{\rho}(z))\right)\|z\| \\
%     &\approx \zeta (B + 1) \mathbb{E}_z\exp(-B||z_1| - |z_2||)\|z\|\\
%     &\approx \zeta.
% \end{align}

% \begin{align}
%     \Delta_2 &\in \pm \mathbb{E}_z \exp(-B(||z_1| - |z_2||)\left(1 - \exp(\zeta (B + 1)\|z\|)\exp(|f_{\rho}(z) - A_{z_1}|z_1| - A_{z_2}|z_2||)\right)\|z\|\\
%     &\in \mathbb{E}_z \exp(-B(||z_1| - |z_2||)\left(1 - \exp(2\zeta (B + 1)\|z\|)\right)\|z\|\\
%     &\in 4\zeta (B + 1)\mathbb{E}_z \exp(-B(||z_1| - |z_2||)\|z\|\\
%     &= \Theta(\zeta),
% \end{align}
% by the lemma below.

% \begin{lemma}
%     \begin{align}
%         \mathbb{E}_z \exp(-B(||z_1| - |z_2||)\|z\| \leq \Theta\left(\frac{1}{B + 1}\right).
%     \end{align}
% \end{lemma}
% \begin{proof}
%         \begin{align}
%         \mathbb{E}_z \exp(-B(||z_1| - |z_2||)\|z\| &\leq \mathbb{E}_r r\mathbb{E}_{\theta} \exp(-Br(||\cos(\theta)| - |\sin(\theta)||)\\
%         &= 8\mathbb{E}_r r\mathbb{E}_{\theta \in [0, \pi/4]} \exp(-Br(\cos(\theta) - \sin(\theta))\\
%         &\leq 8\mathbb{E}_r r\mathbb{E}_{\theta \in [0, \pi/4]} \exp(-Br(1 - 4\theta/\pi))\\
%         &=  8\mathbb{E}_r r\exp(-Br)(\exp(Br) - 1)\frac{\pi}{4Br}\\
%         &= 8\mathbb{E}_r\frac{r}{4}(1 - \exp(-Br))\frac{\pi}{Br}\\
%         &\approx 2\mathbb{E}_r \frac{r}{1 + Br}\\
%         &= \Theta\left(\frac{1}{B + 1}\right)
%     \end{align}
% \end{proof}

% \begin{align}
%     \Delta_2 &= \pm 2\zeta(B + 1)\mathbb{E}_z[\exp(-B||z_1| - |z_2||)\|z\|)\sigma'(z^Tw)z] \leq \zeta.
% \end{align}

% Now
% \begin{align}
%    \mathbb{E}_z[y(z)\exp(-y(z)(A_{z_1}|z_1| - A_{z_2}|z_2|))\sigma'(z^Tw)z] &\approx  \mathbb{E}_z[y(z)\exp(-y(z)(A_{z_1}|z_1| - A_{z_2}|z_2|))\mathbf{1}(z_1 > 0)z]
% \end{align}

% Now 
% \begin{align}
%     \mathbb{E}_z&[y(z)\exp(-A_w||z_1| - |z_2||))\sigma'(z^Tw)z] \approx \mathbb{E}_z[y(z)\exp(-A_w||z_1| - |z_2||))\mathbf{1}(z_1 > 0)z]\\
%     &= \mathbb{E}_z[y(z)\exp(-A_w||z_1| - |z_2||))\mathbf{1}(z_1 > 0)z_1]\\
%     &= \mathbb{E}_{r \sim N(0, 1) > 0}r\mathbb{E}_{\theta \sim [-\pi/2, \pi/2]}y(\theta)\exp(-rA_w(|cos(\theta) - |\sin(\theta)||)\cos(\theta)\\
%     &= 2\mathbb{E}_{r}r\mathbb{E}_{\theta \sim [0, \pi/4]}\exp(-rA_w(cos(\theta) - |\sin(\theta)|)\cos(\theta) -2\mathbb{E}_{r}r\mathbb{E}_{\theta \sim [\pi/4, \pi/2]}\exp(-rA_w(|cos(\theta) - |\sin(\theta)||)\cos(\theta)\\
%     &\approx 2\mathbb{E}_{r}r\mathbb{E}_{\theta \sim [0, \pi/4]}\exp\left(-rA_w\left(1 - \frac{\theta}{\pi/4}\right)\right)\cos(\theta) -2\mathbb{E}_{r}r\mathbb{E}_{\theta \sim [\pi/4, \pi/2]}\exp(-rA_w(|cos(\theta) - |\sin(\theta)||)\cos(\theta)
% \end{align}

% Can do some pairing up argument to ignore the second term. 

% Now 
% \begin{align}
%     \mathbb{E}_{\theta \sim [0, \pi/4]}\exp\left(-rA_w\left(1 - \frac{\theta}{\pi/4}\right)\right)\cos(\theta) &= \exp(-rA_w) \mathbb{E}_{\theta \sim [0, \pi/4]}\exp\left(rA_w\frac{\theta}{\pi/4}\right)\cos(\theta)\\
%     &\approx \exp(-rA_w)\frac{\exp(rA_w)}{1 + rA_w} = \frac{1}{1 + rA_w}.
% \end{align}

% Thus 
% \begin{align}
%     \mathbb{E}_r\frac{r}{1 + rA_w} &\approx \frac{1}{1 + A_w}
% \end{align}

% \end{proof}






\begin{definition}[Strong Neurons for Phase 2]
\begin{enumerate}
    \item $\wsig^{(t)} \in \exp((1 \pm \zeta)/\sqrt{2\pi}t)\wsig^{(0)}$.
    \item $|\wopp^{(t)}| \leq \exp((1 + \zeta)/\sqrt{2\pi}t)|\wopp^{(0)}|$.
    \item $\|\wpe^{(t)}\| \in \exp(\pm \zeta t)\|\wpe^{(0)}\|$.
    \item $a(w) \in \exp(\pm \zeta t)a(w^{0})$
\end{enumerate}
for some $\zeta_1 \in \exp(\pm\Theta(\log\log\log(d)))$ and $\zeta_2 = \Omega(1/log(d)), o(1)$.
\end{definition}
\begin{definition}[Mediocre Neurons for Phase 2]
Let $\cM$ be the set of neurons at such that:
\begin{enumerate}
    \item $\wsig^{(t)} \leq \exp((1 \pm \zeta)/\sqrt{2\pi}t)\wsig^{(0)}$.
    \item $|\wopp^{(t)}| \leq \exp((1 + \zeta)/\sqrt{2\pi}t)|\wopp^{(0)}|$.
    \item $\|\wpe^{(t)}\| \in \exp(\pm \zeta t)\|\wpe^{(0)}\|$.
    \item $a(w) \in \exp(\pm \zeta t)a(w^{0})$
\end{enumerate}
for some $\zeta_1 \in \exp(\pm\Theta(\log\log\log(d)))$ and $\zeta_2 = \Omega(1/log(d)), o(1)$.
\end{definition}
Note that $\cM$ is a super-set of $\cG$. In $\cM$, it is possible that $|\wopp| > |\wsig|$ (in fact $|\wsig|$ can be arbitrarily small), but $|\wopp|$ still cannot be too large - it grows at a most at an exponential rate $\alpha$ smaller than that of $\wsig$ in $\cG$.

We defined $\mathcal{B}$ to be the remaining set of neurons. 

Let $M$ be some large constant. Phase 1 guarantees that $\mathbb{P}_{\hrho_{T_1}}[\hw \in \cG] \geq 1 - \frac{1}{M}$ and $\mathbb{P}_{\hrho_{T_1}}[\hw \in \mathcal{B}] \leq d^{-M}$ for some sufficiently large $M$, and that $\mathbb{E}_{\hrho_{T_1}}[\|\hw\|^2\mathbf{1}(\hw \in \mathcal{B})] \leq d^{-M}$.


The core of this proof the following inductive lemma. We define the following inductive hypothesis.
\begin{definition}[Phase 2 Hypothesis]\label{def:hyp2}
    $\mathbb{P}_{\hrho_{t + T_1}}[\hw \in \mathcal{B}] \leq d^{-M}$ and $\mathbb{E}_{\hrho_{t + T_1}}[\|\hw\|^2\mathbf{1}(\hw \in \mathcal{B})] \leq d^{-M}\exp(4t)$. Suppose also that $\mathbb{P}_{\hrho_{t + T_1}}[\hw \in \cG] \geq 1 - \frac{1}{M}$.
\end{definition}

Let $\eps = \alpha/1000$, and let $T_2 = \sqrt{2\pi}(1 - \eps)\log(d)$.
\begin{lemma}[Phase 2 Inductive Step]\label{lemma:inductive}
Suppose for some $t \leq T_2$, the hypothesis in Defn~\ref{def:hyp2} holds.

Then $\eta \leq 0.1$, and $n \geq d(\log\log(d))^2\log(d)$, with probability at least $1 - d^{-M}$, we have the following:
 \begin{enumerate}
     \item For all $\hw^{(t + T_1)} \in \mathcal{G}$, $\hw^{(t + \eta + T_1)} \in \mathcal{G}.$
     \item For all $\hw^{(t + T_1)} \in \mathcal{M}$, $\hw^{(t + \eta + T_1)} \in \cM.$
     \item $\mathbb{E}_{\hrho_{t + \eta + T_1}}[\|\hw\|^2\mathbf{1}(\hw \in \mathcal{B})] \leq d^{-M}\exp(4(t + \eta)).$
 \end{enumerate}
\end{lemma}

Before proving Lemma~\ref{lemma:inductive}, we make the following observations about implications of the inductive hypothesis. For $z \in \{\pm e_1, \pm e_2\}$, let
\begin{align}
    A_{z} := \mathbb{E}_{\hrho}[\sigma(y(z)a(w)w^Tz)].
\end{align}
We abuse notation and for $v = cz$, for a constant $c$, we define $A_{v} = A_z$.
\begin{claim}\label{claim:inductive}
If Defn~\ref{def:hyp2} holds at some time $t$, we have
    \begin{enumerate}
        \item $B_t := \mathbb{E}_{\hrho_t}[|a(w)|\|w\|)] = o(1)$. 
        \item $\mathbb{E}_{\hrho_t}[\|w_{1:2}\|^2] = o(1)\mathbb{E}_{\hrho_t}[\|\hwpe\|^2]$.
        \item $\mathbb{E}_{\hrho_t}[\|w_{1:2}\|^2] = \frac{\zeta}{d}\exp((1 + o(1))/\sqrt{2\pi}t - 2\alpha t)$.
        \item $\mathbb{E}_{\hrho_t}[\|\hwpe\|^2] = \exp(-2\alpha(1 + o(1))t)$.
        \item $A_z \leq \frac{\zeta_1}{\sqrt{d}}\exp((1 + o(1))/\sqrt{8\pi}t - 2\alpha t)$ for all $z \in \{\pm e_1, \pm e_2\}$
    \end{enumerate}
\end{claim}
\begin{proof}
Simple computation.
\end{proof}

Our main tool in proving Lemma~\ref{lemma:inductive} are the next  two lemmas, concerning the growth of the signal and orthogonal components respectively. Finally, we have a lemma showing that with high probability, the error due to a SGD step with $n = d\log(d)(\log\log(d))^2$ data points is small enough to ignore. Together, these lemmas suffice to show Lemma~\ref{lemma:inductive}.

\begin{lemma}[Phase 2 Signal]\label{lemma:phase2signal}
For any $w$, we have
\begin{align}
    \mathbb{E}_{P}\left[\frac{d}{dt}\wsig^2\right] \in \frac{1}{\sqrt{2\pi}}\left(1 \pm \epsilon_2\right)\wsig^2 \pm |a(w)\wsig|\Theta\left(A_{\wsig}\right).,
\end{align}
    where 
\begin{align}
    \epsilon_2 = \Theta\left(B_t^2 +  \frac{|\wsig| + |\wopp|}{|\wpe| + |\wsig|}\right),
\end{align}

Further, we have 
\begin{align}
    \mathbb{E}_{P}\left[\frac{d}{dt}\wopp^2\right] \in \frac{1}{\sqrt{2\pi}}\left(-1 \pm \epsilon_2\right)\wopp^2 \pm |a(w)\wopp|\Theta\left(A_{\wsig}\right).
\end{align}
Thus assuming the inductive hypothesis, if $w \in \cG$ we have 
\begin{align}
    \mathbb{E}_{P}\left[\frac{d}{dt}\wsig^2\right] = \frac{1}{\sqrt{2\pi}}\left(1 \pm o(1)\right)\wsig^2.
\end{align}
Further, for all $w \in \cM$, we have
\begin{align}
    \mathbb{E}_{P}\left[\frac{d}{dt}\wopp^2\right] \leq \frac{\zeta_1}{d}\exp\left(\left(\frac{1}{\sqrt{2\pi}} + o(1)\right)t -2\alpha t\right)\exp(-2\alpha t),
\end{align}
and 
\begin{align}
    \mathbb{E}_{P}\left[\frac{d}{dt}\wsig^2\right] \leq \frac{1}{\sqrt{2\pi}}\left(1 \pm o(1)\right)\wsig^2.
\end{align}

% $\mathbb{E}_{P}\left[\frac{d}{dt}\hw_2^2\right] \leq \frac{1}{2}\mathbb{E}_{P}\left[\frac{d}{dt}\hw_1^2\right]$.

\end{lemma}

\begin{lemma}[Phase 2 Orthogonal]\label{lemma:phase2orth}
Without regularization, if $\|\hrho\|^2 \leq B_t \leq 0.2$, we have for an individual neuron:
\begin{align}
    \mathbb{E}_{P}\left[\frac{d}{dt}\|\hwpe\|^2\right] \in \pm \Theta(1)a(\hw)\|\hwpe\|\left(\frac{\|w_{1:2}\|}{\|w_{1:2}\| + \|\hwpe\|} + \mathbb{E}_{\hrho}[|a(w)|\sigma(\|w_{1:2}\|)]\right).
\end{align}

Thus assuming the inductive hypothesis of Phase 2 and that $\|\hw_{1:2}\| = o(1)\|\hwpe\|$ (which in particular holds for any $\hw \in \cM$), we have
\begin{align}\label{eq:perp}
\frac{d}{dt}\mathbb{E}[\|\hwpe\|^2] = o(1)\mathbb{E}[\|\hwpe\|^2].
\end{align}
\end{lemma}

Let 
\begin{align}
    \delta_1 &:= \mathbb{E}_{\rho}[\|\wpe^{(0)} - \wpe^{(t)}\|^2]\\
    \delta_2 &:= \mathbb{E}_{\rho}[(a(w^{(0)}) - a(w^{(t)}))^2]\\
\end{align}
% \begin{lemma}[Alternative Orthogonal.]\label{lemma:alt}
% For any individual neuron in $\cM$, we have whp:

% \begin{align}
%     \|\mathbb{E}_{x \sim P_n}[\nabla L(x; \wpe)]\| \leq |a(w)|(1 + 5B_t)\left(\sqrt{\frac{d}{n}} + B_t\right).
% \end{align}

% Further, we have whp:
% \begin{align}
%     |\mathbb{E}_{x \sim P_n}[\nabla L(x; a(w))]| \leq \|w\|\left(B_t + \frac{1}{\sqrt{n}}\right).
% \end{align}

% \end{lemma}
% \begin{corollary}
% For any individual neuron in $\cM$, we have whp for the duration of $T_2$ that if $B_t < \frac{1}{2}$, then
% \begin{align}
%     a(w^{(t)}) \in a(w^{(0)})(1 \pm \zeta);
% \end{align}
% \begin{align}
%     \|w^{(t)}\| \in \|w^{(0)}\|(1 \pm \zeta);
% \end{align}
% \end{corollary}
% \begin{proof}[Proof of Lemma~\ref{lemma:alt}]
%     \begin{align}
%         \|\mathbb{E}_{x \sim P_n}[\nabla L(x; \wpe)]\|^2 &= a(w)^2\frac{1}{n^2}\sum_{i, j \in [n]} \ell'_{\rho}(x_i)\ell'_{\rho}(x_j)\sigma'(w^Tx_i)\sigma'(w^Tx_j)x_i^Tx_j\\
%         &= a(w)^2\frac{1}{n^2}\sum_{i, j \in [n]} (\ell'_{\rho}(x_i))^2\sigma'(w^Tx_i)\|x_i\|^2\\
%         &\qquad + a(w)^2\frac{1}{n^2}\sum_{i \neq j} \ell'_{\rho}(x_i)\ell'_{\rho}(x_j)\sigma'(w^Tx_i)\sigma'(w^Tx_j)x_i^Tx_j\\
%         &\leq a(w)^2\frac{d}{n}\exp(2B_t) + a(w)^2\frac{1}{n^2}\sum_{i \neq j} \ell'_{\rho}(x_i)\ell'_{\rho}(x_j)\sigma'(w^Tx_i)\sigma'(w^Tx_j)x_i^Tx_j\\
%     \end{align}

% Now letting $\Delta_i := |y(x_i) - \ell'_{\rho}(x_i)|$, we have with high probability that
% \begin{align}
%     \sum_{i \neq j} \ell'_{\rho}(x_i)\ell'_{\rho}(x_j)\sigma'(w^Tx_i)\sigma'(w^Tx_j)x_i^Tx_j &\leq \sum_{i \neq j} y(x_i)y(x_j)\sigma'(w^Tx_i)\sigma'(w^Tx_j)x_i^Tx_j\\
%     &\quad + \sup_{v \in \mathbb{R}^n, \|v\|^2 \leq \sum_i \Delta_i^2} v^TX^TXv\\
%     &\leq \sqrt{d}n  + (\exp(\delta_1\sqrt{\mathbb{E}_{\rho}[a(w)^2]} + \delta_2\sqrt{\mathbb{E}_{\rho}[\|w\|^2]}) - 1)^2 n^2.
% \end{align}
% Here the last inequality is the part that holds with high probability.

% Thus with high probability, assuming $\delta_1, \delta_2 \ll 1$ we have
% \begin{align}
%     \frac{1}{a(w)^2}\|\mathbb{E}_{x \sim P_n}[\nabla L(x; \wpe)]\|^2 &\leq \frac{d}{n}\exp(2B_t) + \delta_1^2\mathbb{E}_{\rho}[a(w)^2] + \delta_2^2\mathbb{E}_{\rho}[\|w\|^2],
% \end{align}
% or for $B_t \leq 1$,
% \begin{align}
%     \|\mathbb{E}_{x \sim P_n}[\nabla L(x; \wpe)]\| \leq |a(w)|(1 + 5B_t)\left(\sqrt{\frac{d}{n}} + \delta_1\sqrt{\mathbb{E}_{\rho}[a(w)^2]} + \delta_2\sqrt{\mathbb{E}_{\rho}[\|w\|^2]}\right)
% \end{align}

% For the second part, we have
% \begin{align}
%     |\mathbb{E}_{x \sim P_n}[\nabla L(x; a(w))]| &= |\frac{1}{n}\sum_{i = 1}^n \ell'_{\rho}(x_i)\sigma(w^Tx_i)|\\
%     &\leq |\frac{1}{n}\sum_{i = 1}^n y(x_i)\sigma(w^Tx_i)| + \frac{1}{n}\sum_{i = 1}^n \Delta_i\sigma(w^Tx_i)\\
%     &\leq \|w\|_2\Theta\left(\frac{1}{\sqrt{n}}\right) + \frac{1}{n}\|w^TX\|_2\|\Delta\|_2\\
%     &\leq  \|w\|_2\Theta\left(\frac{1}{\sqrt{n}}\right) + \|w\|_2\left(\delta_1\sqrt{\mathbb{E}_{\rho}[a(w)^2]} + \delta_2\sqrt{\mathbb{E}_{\rho}[\|w\|^2]}\right)
% \end{align}
% \end{proof}

% Let $L_y$ denote the loss function where $\ell'_{\rho}(x) = -y(x)$ always.
% \begin{lemma}\label{lemma:approxsig}
%     For any individual neuron in $w \in \cM$, we have whp:
%     \begin{align}
%         |\mathbb{E}_{x \sim P_n}[\nabla L_{\rho}(x; \wsig)] - \mathbb{E}_{x \sim D}[\nabla L_{y}(x; \wsig)]| \leq \zeta \mathbb{E}_{x \sim D}[\nabla L_{y}(x; \wsig)].
%     \end{align}
% \end{lemma}
% \begin{proof}
%     We break this up into two pieces:
%     \begin{align}
%         |\mathbb{E}_{x \sim P_n}[\nabla L_{\rho}(x; \wsig)] - \mathbb{E}_{x \sim D}[\nabla L_{\rho}(x; \wsig)]|,
%     \end{align}
%     and 
%     \begin{align}
%         |\mathbb{E}_{x \sim D}[\nabla L_{\rho}(x; \wsig)] - \mathbb{E}_{x \sim D}[\nabla L_{y}(x; \wsig)]|.
%     \end{align}
% The first term is easy to control through standard concentration tools. 

% For the second term, we leverage the symmetry of the data. Let $\Delta_{\xi, z} := |\exp(-f(\xi + z)) - \exp(-f(\xi))|$.
% \begin{align}
%     \frac{1}{a(w)}\mathbb{E}_{x \sim D}[\nabla L_{\rho}(x; \wsig)] &= \mathbb{E}_{x \sim D}[\ell'_{\rho}(x)\sigma'(w^Tx)z]\\
%     &= \mathbb{E}_{\xi, z \sim D}[-y(z)\exp(-f(\xi + z))\sigma'(w^T\xi + w^Tz)z]\\
%     &\in  \mathbb{E}_{\xi, z \sim D}[-y(z)\exp(-f(\xi))\sigma'(w^T\xi + w^Tz)z] \pm  \mathbb{E}_{\xi, z \sim D}[\Delta_{\xi, z}\sigma'(w^T\xi + w^Tz)\|z\|]v,
% \end{align}
% where $v$ is any unit vector.

% Now fix some $z$, and let $\phi$ be drawn from the symmetry group of $z$. Let $\Delta_{\xi} := |f(\xi)|$. We have
% \begin{align}
%     \mathbb{E}_{r \in \pm 1}&\mathbb{E}_{\xi}[-y(rz)\exp(-f(\xi))\sigma'(w^T\xi + rw^Tz)rz]= 
%     \mathbb{E}_{\xi}[-y(z)\exp(-f(\xi))\mathbf{1}(|w^T\xi| \leq |w^Tz|)z\on{sign}(w^Tz)]\\
%     &= \mathbb{E}_{r\sim \pm 1}\mathbb{E}_{\xi}[-y(rz)\sigma'(w^T\xi + rw^Tz)z] \pm \mathbb{E}_{\xi}[\Delta_{\xi}\mathbf{1}(|w^T\xi| \leq |w^Tz|)\|z\|]v,
% \end{align}
% where $v$ is any unit vector. Now by lemma \mg{BLAH}, we have 
% \begin{align}
%     \mathbb{E}_{\xi}[\Delta_{\xi}\mathbf{1}(|w^T\xi| \leq |w^Tz|)\|z\|] \leq \Theta(1)B_t \frac{\|w_{1:2}\|}{\|w\|}.
% \end{align}

% \end{proof}

\section{Old Phase 2 $\wns$ analysis}

\begin{claim}[Clean Population Gradients for $\wpe$]\label{claim:wpe}
\begin{align}
    -\wpe^T\ncl L(w) \leq \begin{cases}
        -4 \zeta H \|\wpe\| |a(w)| & \|\wpe\| \geq \zeta \|\wsig\|/2\\
        \|\wpe\|^2\frac{\tau}{4}\exp(-\bmu)\frac{|a(w)|}{\|\wsig\|} & \text{otherwise}.
    \end{cases} 
\end{align}
\end{claim}
\begin{proof}[Proof of Claim~\ref{claim:wpe}]

\begin{align}
    \mathbb{E}_x \ell'_{\rho}(z)\sigma'(w^Tx)x^T\wpe &= \mathbb{E}_{\xi}\mathbb{E}_z \ell'_{\rho}(z)\sigma'(w^T\xi + w^Tz)\xi^T\wpe\\
    &= \frac{1}{2}\mathbb{E}_{\xi}\mathbb{E}_z \ell'_{\rho}(z)\left(\sigma'(w^T\xi + w^Tz) - \sigma'(-w^T\xi + w^Tz)\right)\xi^T\wpe\\
    &=\frac{1}{2}\mathbb{E}_z \ell'_{\rho}(z)  \mathbb{E}_{\xi}\mathbf{1}(|w^T\xi| \geq |w^Tz|)|\xi^T\wpe|,
\end{align}

Now 
\begin{align}
    -\on{sign}(a(w))\mathbb{E}_z \ell'_{\rho}(z)  \mathbb{E}_{\xi}\mathbf{1}(|w^T\xi| \geq |w^Tz|)|\xi^T\wpe| &\leq \frac{1}{4}\exp(-\bmin)\mathbb{E}_{\xi}\mathbf{1}(|w^T\xi| \geq |w^T\mu|)|\xi^T\wpe|\\
    &\quad - \frac{1}{4}\exp(-\bmax)\mathbb{E}_{\xi}\mathbf{1}(|w^T\xi| \geq \sqrt{2}\|\wopp\|)|\xi^T\wpe|\\
\end{align}



For the second term, if $\|\wpe\| \geq \zeta \|\wsig\|/2$, then by our inductive hypothesis, we have $\|\wpe\| \geq \|\wopp\|/(2\sqrt{2H})$, and so


\begin{align}
    \exp(-\bmax)\mathbb{E}_{\xi}\mathbf{1}(|w^T\xi| \geq \sqrt{2}\|\wopp\|)|\xi^T\wpe| &\geq \exp(-\bmax)\|\wpe\|\exp(-\|\wopp\|^2/\|\wpe\|^2)\\
    &\geq  \exp(-\bmax)\|\wpe\|\exp(-8H)\\
    &\geq 2\zeta H \|\wpe\|,
\end{align}
because 
\begin{align}
    \exp(-8H) \geq 3 H \exp(H)\zeta,
\end{align}
since by assumption, we have $\log(1/\zeta) \geq 10 H$. 


% Thus we have 
% \begin{align}
%     \|\wpe^{(t + 1)}\|^2 &\leq \|\wpe^{(t)}\|^2 - 2\eta a(w)\mathbb{E}_x \ell'_{\rho}(x)\sigma'(w^Tx)x^T\wpe + \eta^2a(w)^2 \|\mathbb{E}_x \ell'_{\rho}(x)\sigma'(w^Tx)\xi\|^2\\
%     &\leq \|\wpe^{(t)}\|^2 + 2\eta \sqrt{\frac{1}{8\pi}}\exp(-B)\|\wpe\|\frac{\|\wpe\|}{\|w\|}|a(w)| + 4\eta \exp(-B) \|\wpe\| |a(w)| \zeta B\\
%     &\qquad + \eta^2 a(w)^2 \exp(-2B)\left(\frac{1}{8\pi} + \frac{d}{n}\right)\frac{\|\wpe\|^2}{\|w\|^2}\\
%     &\leq  \|\wpe^{(t)}\|^2\left(1 +  2\eta \sqrt{\frac{1}{8\pi}}\exp(-B) + \eta^2 \frac{1}{8\pi}\exp(-2B)\right).
% \end{align}

% Here we have used Lemma~\ref{lemma:layer_balance} to bound $|a(w)|$ by $\|w\|$.
\end{proof}
\begin{claim}[Clean Population Gradients for $\wopp$]\label{claim:wopp}
\begin{align}
    - \wopp^T\ncl L(w) \leq \begin{cases}
         -4\zeta H \|\wopp\||a(w)| &\|\wopp\| \geq \sqrt{1.5H}\zeta \|\wsig\|\\
         \frac{\sqrt{2}\|\wopp\|}{4}\exp(-\bmin)|a(w)| & \text{otherwise}.
     \end{cases}
\end{align}
\end{claim}
\begin{proof}[Proof of Claim~\ref{claim:wopp}]

\begin{align}
     -\on{sign}(a(w))\mathbb{E}_x \ell'_{\rho}(z)\sigma'(w^Tx)x^T\wopp &\leq \frac{1}{4}\mathbb{E}_{\xi} \exp(-\bmin)\mathbf{1}(|w^T\xi| \geq \sqrt{2}\|\wopp\|)\sqrt{2}\|\wopp\| \\
     &\qquad -  \frac{1}{8}\exp(-\bmax)\sqrt{2}\|\wopp\|.
\end{align}

Now if $\|\wopp\| \geq \sqrt{1.5H}\zeta \|\wsig\|$, then $\|\wopp\| \geq \sqrt{1.5H}\|\wopp\|$, and so 
\begin{align}
    \mathbb{P}[|w^T\xi| \geq \sqrt{2}\|\wopp\|] \leq \exp(-1.5H) \leq 8\exp(-\bmax),
\end{align}
and thus 
\begin{align}
    -\on{sign}(a(w))\mathbb{E}_x \ell'_{\rho}(z)\sigma'(w^Tx)x^T\wopp &\leq  -\frac{1}{10}\exp(-\bmax)\sqrt{2}\|\wopp\|\\
    &\geq 4\zeta H \|\wopp\|.
\end{align}

Otherwise, we have (trivially) that
\begin{align}
    -\on{sign}(a(w))\mathbb{E}_x \ell'_{\rho}(z)\sigma'(w^Tx)x^T\wopp &\leq \frac{\sqrt{2}}{4}\exp(-\bmin)\|\wopp\|.
\end{align}

\end{proof}

We can now combine Claims~\ref{claim:wsig}, \ref{claim:wpe}, \ref{claim:wopp}, and Lemma~\ref{claim:approxerror} to prove that we maintain the inductive hypothesis after one minibatch SGD step. Indeed, for $w \in S_{\mu}$, we have:
\begin{enumerate}
    \item $\|\wsig^{(t + 1)}\| \geq \|\wsig^{(t)}\|$.
    \item Since $\eta$ is small enough (relative to $\zeta$), if $\|\wpe^{(t)}\| \leq \zeta \|\wsig^{(t)}\|/2$, then $\|\wpe^{(t + 1)}\| \leq \zeta \|\wsig^{(t)}\| \leq \zeta \|\wsig^{(t + 1)}\|$.
    \item Similarly, since $\eta$ is small enough, if $\|\wopp^{(t)}\| \leq \zeta \|\wsig^{(t)}\|\sqrt{1.5H}$, then $\|\wopp^{(t + 1)}\| \leq \zeta \|\wsig^{(t)}\|\sqrt{2H} \leq \zeta \|\wsig^{(t + 1)}\|\sqrt{2H}$.
    \item If $\|\wpe^{(t)}\| \geq \zeta \|\wsig^{(t)}\|/2$, then 
    \begin{align}
        \|\wpe^{(t + 1)}\|^2 &\leq \|\wpe^{(t)}\|^2 -2\eta (\wpe^{(t)})^T\nabla \hat{L}(w) + \eta^2 \|\nabla \hat{L}(w) \|^2\\
        &\leq  \|\wpe^{(t)}\|^2 -2\eta (\wpe^{(t)})^T\ncl L(w) + 2\eta \|\wpe\|\|\nabla \hat{L}(w) - \ncl L(w)\| + \eta^2 \|\nabla \hat{L}(w) \|^2\\
        &\leq \|\wpe^{(t)}\|^2 -2\eta |a(w)|\|\wpe\|4\zeta H + 2\eta \|\wpe\|2\zeta H |a(w)| + \eta^2 \|\nabla \hat{L}(w) \|^2\\
        &=  \|\wpe^{(t)}\|^2 - 4\eta |a(w)|\|\wpe\|\zeta H + \eta^2 \|\nabla \hat{L}(w)\|^2\\
        &\leq  \|\wpe^{(t)}\|^2 - 4\eta |a(w)|\|\wpe\|\zeta H + \eta^2L^2 a(w)^2\\
        &\leq  \|\wpe^{(t)}\|^2 - 4\eta |a(w)|\|\wpe\|\zeta H + 2\eta^2L^2 |a(w)|\|\wsig\|\\
        &\leq  \|\wpe^{(t)}\|^2 - 4\eta |a(w)|\|\wpe\|\zeta H + 2\eta^2L^2 |a(w)|\|\wpe\|/\zeta \\
        &\leq \|\wpe^{(t)}\|^2\\
        &\leq \zeta^2\|\wsig^{(t + 1)}\|^2.
    \end{align}
    where in the second to last inequality we used the fact that $\eta \leq \zeta^2$. 
    \item  If $\|\wopp^{(t)}\| \geq \zeta \sqrt{2H}\|\wsig^{(t)}\|/2$, then by a similar argument,
    \begin{align}
        \|\wopp^{(t + 1)}\|^2 &\leq \|\wopp^{(t)}\|^2 -2\eta (\wopp^{(t)})^T\nabla \hat{L}(w) + \eta^2 \|\nabla \hat{L}(w) \|^2\\
        &\leq  \|\wopp^{(t)}\|^2 -2\eta (\wopp^{(t)})^T\ncl L(w) + 2\eta \|\wopp\|\|\nabla \hat{L}(w) - \ncl L(w)\| + \eta^2 \|\nabla \hat{L}(w) \|^2\\
        &\leq \|\wopp^{(t)}\|^2 - 4\eta |a(w)|\|\wopp\| \zeta H + \eta^2 \|\nabla \hat{L}(w)\|^2 \\
        &\leq  \|\wopp^{(t)}\|^2- 4\eta |a(w)|\|\wopp\| \zeta H + 2\eta^2L^2 |a(w)|\|\wpe\|/\zeta \\
        &\leq  \|\wopp^{(t)}\|^2 \\
        &\leq 2H\zeta^2\|\wsig^{(t + 1)}\|^2.
        \end{align}
\end{enumerate}

